Multiple protein feature prediction with statistical relational learning

High throughput sequencing techniques have highly impactedon modern biology, widening the gap between sequenced andannotated data. Automatic annotation tools are thereforeof the foremost importance to guide biologists' experiments. However, most of the state-of-the-art methods rely on annotation transfer, offering reliable predictions only in homology settings. In this work we present a novel appraoch to protein feature prediction, which exploits the Semanti Based Regularization to inject prior knowledge in the learning process. The experimental results conducted on the yeast genome show that the introduction of the constraints positively impacts on the overall prediction quality.

==> abstract/abstract.tex <==
\addcontentsline{toc}{chapter}{Abstract}

\begin{abstract}

Text of the Abstract.

\end{abstract}

==> acknowledgements/acknowledgements.tex <==
\cleardoublepage

\addcontentsline{toc}{chapter}{Acknowledgements}

\begin{acknowledgements}

I would like to express (whatever feelings I have) to:

\begin{itemize}
 \item My supervisor
 \vspace*{3mm}
 \item My second supervisor
 \vspace*{3mm}
 \item Other researchers
 \vspace*{3mm}
 \item My family and friends
\end{itemize}

\end{acknowledgements}

==> figures/out.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(9070.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,440){\makebox(0,0)[r]{\strut{} 0.55}}%
      \put(858,777){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(858,1114){\makebox(0,0)[r]{\strut{} 0.65}}%
      \put(858,1451){\makebox(0,0)[r]{\strut{} 0.7}}%
      \put(858,1788){\makebox(0,0)[r]{\strut{} 0.75}}%
      \put(858,2124){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(858,2461){\makebox(0,0)[r]{\strut{} 0.85}}%
      \put(858,2798){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(858,3135){\makebox(0,0)[r]{\strut{} 0.95}}%
      \put(990,220){\makebox(0,0){\strut{} 2}}%
      \put(2271,220){\makebox(0,0){\strut{} 2.5}}%
      \put(3551,220){\makebox(0,0){\strut{} 3}}%
      \put(4832,220){\makebox(0,0){\strut{} 3.5}}%
      \put(6112,220){\makebox(0,0){\strut{} 4}}%
      \put(7393,220){\makebox(0,0){\strut{} 4.5}}%
      \put(8673,220){\makebox(0,0){\strut{} 5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(7686,1273){\makebox(0,0)[r]{\strut{}interpro}}%
      \csname LTb\endcsname%
      \put(7686,1053){\makebox(0,0)[r]{\strut{}microarray}}%
      \csname LTb\endcsname%
      \put(7686,833){\makebox(0,0)[r]{\strut{}spectrum}}%
      \csname LTb\endcsname%
      \put(7686,613){\makebox(0,0)[r]{\strut{}complex}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{out}}%
    \gplfronttext
  \end{picture}%
\endgroup

==> figures/prova2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(8502.00,3770.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(990,440){\makebox(0,0)[r]{\strut{} 0.88}}%
      \put(990,823){\makebox(0,0)[r]{\strut{} 0.885}}%
      \put(990,1206){\makebox(0,0)[r]{\strut{} 0.89}}%
      \put(990,1589){\makebox(0,0)[r]{\strut{} 0.895}}%
      \put(990,1973){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(990,2356){\makebox(0,0)[r]{\strut{} 0.905}}%
      \put(990,2739){\makebox(0,0)[r]{\strut{} 0.91}}%
      \put(990,3122){\makebox(0,0)[r]{\strut{} 0.915}}%
      \put(990,3505){\makebox(0,0)[r]{\strut{} 0.92}}%
      \put(1122,220){\makebox(0,0){\strut{} 2}}%
      \put(2868,220){\makebox(0,0){\strut{} 2.5}}%
      \put(4614,220){\makebox(0,0){\strut{} 3}}%
      \put(6359,220){\makebox(0,0){\strut{} 3.5}}%
      \put(8105,220){\makebox(0,0){\strut{} 4}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(7118,3332){\makebox(0,0)[r]{\strut{}"data.dat" using 1:2}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{prova2}}%
    \gplfronttext
  \end{picture}%
\endgroup

==> methods/sbrs_parameters.tex <==
\section{SBR version and parameters}
SBR is an ongoing project that is constantly developed and updated. In this work we had the need/occasion to use two very different version of the software because the first version accepted only the constraints in Conjunctive Normal Form (CNF), while the DPP constraints are in Disjunctive Normal Form (DNF) and the conversion to CNF would make them exponentially longer. Unfortunately the second version has been made available only in the last days of work and therefore the first experiments done could not been re executed on that version. 

In this section we will show the common parameters and the different and explain why the experiments results obtained with the two version of the code are biased and therefore not completely comparable.

\subsubsection{SBR Conjunctive Normal Form}
\begin{itemize}
\item weights:
\item transductive:
\item t-norms:
\end{itemize}


\subsubsection{SBR 6.0}
\begin{itemize}
\item 
\end{itemize}

